Long-time turbulence prediction at fine time steps using multi-stride neural operators

Long-time turbulence prediction at fine time steps is costly and prone to error accumulation, while accurate short-term fields do not ensure accurate long-time statistics. We propose a multi-stride neural operator for three-dimensional turbulence, combining implicit factorized Transformer (IFF) predictors with a factorized-attention cross-stride fusion (FA-CSF) module. All predictors take the same current velocity field as input. FA-CSF reuses their outputs and latent features to generate intermediate velocity fields through interpolation and learned correction. The corrected largest-stride field drives the next autoregressive step, decoupling the autoregressive step from the output time step. Stride-conditioned IFF (SC-IFF) predictors are first trained at power-of-two strides using three conditioning strategies, then frozen while FA-CSF is trained on long rollouts with field-data and statistical losses. Tests on turbulent channel flow and forced homogeneous isotropic turbulence (HIT) show improved long-time predictions and statistics. At a sampling interval of 10 direct numerical simulation (DNS) time steps, fixed-stride IFF yields relative L2 errors above 100% in channel-flow root-mean-square (RMS) velocity fluctuation profiles and the Reynolds shear stress profile, and in the temporal evolution of velocity and vorticity RMS values and the time-averaged energy spectrum in HIT. SC-IFF with independent stride-specific predictors and FA-CSF keeps statistics close to filtered DNS data over the tested prediction times. Relative to fixed-stride IFF, it reduces errors in the channel-flow profiles by more than 98% and in the HIT spectrum by more than 99%. Multi-stride prediction with FA-CSF generates trajectories at fine time steps 3.69 times faster than fixed-stride IFF autoregression and 2.41 times faster than hierarchical multi-stride prediction.

==> figure/method/method_figure_style.tex <==
\ifdefined\MFbox\else\newsavebox{\MFbox}\fi
\definecolor{MFLearned}{HTML}{DCE8F4}
\definecolor{MFAttention}{HTML}{F4DFB9}
\definecolor{MFAttnDark}{HTML}{C98A2B}
\definecolor{MFEncode}{HTML}{E6DDF1}
\definecolor{MFFixed}{HTML}{EDEEEF}
\definecolor{MFIFF}{HTML}{2F6690}
\definecolor{MFIFFFill}{HTML}{F2F7FB}
\definecolor{MFCSF}{HTML}{2D7A57}
\definecolor{MFCSFFill}{HTML}{EFF7F2}
\definecolor{MFGrad}{HTML}{B03A2E}
\definecolor{MFFrame}{HTML}{BCC1C6}
\definecolor{MFField}{HTML}{D2DFEB}
\definecolor{MFFieldTop}{HTML}{E8EFF6}
\definecolor{MFFieldSide}{HTML}{A7BBCD}
\definecolor{MFLatent}{HTML}{E4E4E4}
\definecolor{MFLatentTop}{HTML}{F2F2F2}
\definecolor{MFLatentSide}{HTML}{BDBDBD}
\def\MFfont{\fontsize{8.5}{10}\selectfont}
\def\MFsmall{\fontsize{7.6}{9}\selectfont}
\def\MFtitlefont{\fontsize{9.5}{11.5}\selectfont\bfseries}
\tikzset{
  mf/.style={x=1cm,y=1cm,>={Latex[length=1.6mm,width=1.2mm]},
    every node/.style={font=\MFfont,inner sep=1.5pt}},
  mfop/.style={draw=black!55,line width=.5pt,rounded corners=1.5pt,align=center,
    inner xsep=3pt,inner ysep=2pt,minimum height=.62cm,fill=MFFixed},
  mflearn/.style={mfop,fill=MFLearned},
  mfattn/.style={mfop,fill=MFAttention},
  mfenc/.style={mfop,fill=MFEncode},
  mffixed/.style={mfop},
  mfdata/.style={mfop,fill=white},
  mfiff/.style={draw=MFIFF,line width=.85pt,rounded corners=2.5pt,fill=MFIFFFill},
  mfcsf/.style={draw=MFCSF,line width=.85pt,rounded corners=2.5pt,fill=MFCSFFill},
  mfgroup/.style={draw=MFFrame,line width=.5pt,rounded corners=2.5pt},
  mfflow/.style={->,line width=.6pt},
  mfwire/.style={line width=.6pt},
  mfloop/.style={->,line width=.6pt,dash pattern=on 2.2pt off 1.5pt},
  mfgrad/.style={->,draw=MFGrad,line width=.7pt,dash pattern=on 2.6pt off 1.6pt},
  mfadd/.style={draw=black!60,circle,fill=white,minimum size=.36cm,inner sep=0pt,line width=.5pt},
  mftitle/.style={anchor=west,font=\MFtitlefont,inner sep=0pt},
  mfhead/.style={font=\fontsize{8.5}{10}\selectfont\bfseries,inner sep=1pt},
  mfnote/.style={font=\MFsmall,align=center,inner sep=1pt,text=black!80},
  mfshape/.style={font=\MFsmall,text=black!66,inner sep=1pt},
  mfvar/.style={inner sep=1.5pt},
  mfbridge/.style={preaction={draw=white,line width=2.8pt}},
  mfswatch/.style={draw=black!55,line width=.45pt,rounded corners=1pt,minimum width=.42cm,minimum height=.26cm,inner sep=0pt},
}
\providecommand{\MFdot}[1]{\fill #1 circle (.9pt);}
\providecommand{\MFsnow}[2]{%
  \begin{scope}[shift={#1},draw=MFIFF,line width=.42pt,line cap=round]
    \foreach \MFa in {0,60,120}{\draw[rotate=\MFa] (-#2,0)--(#2,0);}
    \foreach \MFa in {0,60,...,300}{\draw[rotate=\MFa]
      (.58*#2,0)--++(45:.36*#2) (.58*#2,0)--++(-45:.36*#2);}
  \end{scope}}
\providecommand{\MFcube}[3]{%
  \begin{scope}[shift={#1},line width=.4pt,draw=black!62]
    \path[draw,fill=#3] (-#2,-#2) rectangle (#2,#2);
    \path[draw,fill=#3Top] (-#2,#2)--(-.35*#2,1.65*#2)--(1.65*#2,1.65*#2)--(#2,#2)--cycle;
    \path[draw,fill=#3Side] (#2,-#2)--(1.65*#2,-.35*#2)--(1.65*#2,1.65*#2)--(#2,#2)--cycle;
  \end{scope}}
\providecommand{\MFoutput}{%
  \ifdim\wd\MFbox>\linewidth\resizebox{\linewidth}{!}{\usebox{\MFbox}}\else\usebox{\MFbox}\fi}

